Towards a Comprehensive Human-Centred Evaluation Framework for Explainable AI

While research on explainable AI (XAI) is booming and explanation techniques have proven promising in many application domains, standardised human-centred evaluation procedures are still missing. In addition, current evaluation procedures do not assess XAI methods holistically in the sense that they do not treat explanations' effects on humans as a complex user experience. To tackle this challenge, we propose to adapt the User-Centric Evaluation Framework used in recommender systems: we integrate explanation aspects, summarise explanation properties, indicate relations between them, and categorise metrics that measure these properties. With this comprehensive evaluation framework, we hope to contribute to the human-centred standardisation of XAI evaluation.

==> tables/metrics/MetricsAbstraction.tex <==
\begin{tabularx}{\linewidth}{@{}p{3.5cm}X@{}}
  \toprule
  \textbf{Explanation property} & Measurements  \\
  \midrule
  
  Certainty & Confidence Accuracy \cite{Nauta2022FromAI}  \\
   
  Continuity &  Connectedness \cite{Nauta2022FromAI} also in \cite{Singh2022ExplainabilityMethods, MoraffahCausalEvaluation, Moreira2022BenchmarkingBox, Vilone2021NotionsIntelligence, Ge2021CounterfactualAI, Carlevaro2022CounterfactualDescription}; Stability for Slight Variations \cite{Nauta2022FromAI}; Fidelity for Slight Variations \cite{Nauta2022FromAI}  \\

  Separability & Separability \cite{Carvalho2019MachineMetrics} \\

  Consistency & Stability of explanation: check whether the explanations for a single object change for different instances of the XAI method \cite{Coroama2022EvaluationXAI, Carvalho2019MachineMetrics} \\
  \hline
  Necessity & Responsability of an outcome \cite{Miller2019}; Sparsity and Sparsity rate \cite{Moreira2022BenchmarkingBox}; Deletion Check \cite{Nauta2022FromAI, Li2022AMetrics} \\

  Sufficiency & Count whether the AI model prediction changes when the non-selected causes change \cite{Miller2019} \\
  
  Correctness &  Model Parameter Randomization Check, Explanation Randomization, White Box Check, Controlled Synthetic Data Check, Predictive Performance \cite{Nauta2022FromAI}; Fidelity  \cite{Sokol2020ExplainabilityApproaches, Coroama2022EvaluationXAI, Nauta2022FromAI}; Alignment between AI model features and explanation features \cite{Li2022AMetrics, Velmurugan2021DevelopingLearning}\\

  Completeness & Preservation Check \cite{Nauta2022FromAI}; Completeness \cite{Coroama2022EvaluationXAI, MoraffahCausalEvaluation}; Recall \cite{Velmurugan2021DevelopingLearning}  \\

  Contrastivity & Data Randomization, Target Sensitivity, Target Dicriminativeness \cite{Nauta2022FromAI}; Sensitivity \cite{Vilone2021NotionsIntelligence} \\

  Size & Total size or sparsity \cite{Nauta2022FromAI} \\
  
  Structure & Incremental Deletion \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Covariate Regularity \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Chronology \cite{Sokol2020ExplainabilityApproaches}; Single Deletion \cite{Nauta2022FromAI} \\

  Representativeness & Explanation support (number of instances to which the explanation applies over the number of instances) \cite{Sokol2020ExplainabilityApproaches, Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence, Coroama2022EvaluationXAI} \\
  
    \hline 

    Explanation power & Sensitivity Axiom \cite{Carvalho2019MachineMetrics}\\

    Form of cognitive chunks & Covariate Homogeneity \cite{Nauta2022FromAI} \\

    Information expectedness & Alignment with Domain Knowledge \cite{Nauta2022FromAI} \\

   
    Relevance to the task & Pragmatism \cite{Nauta2022FromAI, Coroama2022EvaluationXAI, Moreira2022BenchmarkingBox}; Attribute costs \cite{Vilone2021NotionsIntelligence} \\
    
  
  \bottomrule
\end{tabularx}


==> tables/metrics/MetricsCommunication.tex <==
\begin{tabularx}{\linewidth}{@{}p{3.5cm}X@{}}
  \toprule
  \textbf{Explanation property} & Measurement \\ 
  \midrule
  Structure & Questionnaire \cite{Vilone2021NotionsIntelligence, Chen2005TrustAgents} \\
\hline
  Explanation power &  Questionnaire \cite{Vilone2022AIntelligence}\\

    Form of cognitive chunks &  Perceived Homogeneity \cite{Nauta2022FromAI} \\

    Information expectedness &  Questionnaire \cite{Vilone2022AIntelligence}\\
    
    Perceived model competence &  Questionnaire \cite{Ashoori2019InProcesses}\\

    Cognitive Load &  NASA TLX \cite{Hsiao2021RoadmapXAI}\\
   
    Relevance to the task &  Questionnaire \cite{Vilone2022AIntelligence}\\
    
    Alignment with situational context & Goodness explanation \cite{Hoffman2018MetricsProspects} \\
    \hline
    Curiosity & Curiosity Checklist \cite{Hoffman2018MetricsProspects}; Eye Movement Pattern \cite{Hsiao2021RoadmapXAI} \\

    Satisfaction & Explanation Satisfaction Scale \cite{Hoffman2018MetricsProspects}; Eye Movement Pattern \cite{Hsiao2021RoadmapXAI}; Loyalty \cite{Tintarev2015ExplainingEvaluation}; Questionnaire \cite{Ashoori2019InProcesses} \\
  
    Trust & Trust Scale \cite{Hoffman2018MetricsProspects}; Questionnaire \cite{Ashoori2019InProcesses, Chen2005TrustAgents, Pu2007Trust-inspiringSystems, Vilone2022AIntelligence}\\

    Understanding & Questionnaires \cite{Tintarev2015ExplainingEvaluation,Ashoori2019InProcesses, Vilone2022AIntelligence}\\

    Helpfulness & Questionnaires \cite{Tintarev2015ExplainingEvaluation, Vilone2022AIntelligence}; Evaluate user action before and after explanation \cite{Tintarev2015ExplainingEvaluation}\\

    Controllability & Concept-level feedback Satisfaction Ratio \cite{Chen2020TowardsRecommendation}; The extent to which a user can produce certain outcomes \cite{Hoffman2018MetricsProspects}\\
    \hline Efficiency & Interaction time and number of interactions to perform a task \cite{Tintarev2015ExplainingEvaluation}\\
    
    Performance & Performance metrics with respect to the primary goal \cite{Hoffman2018MetricsProspects} \\
    
    Reliance & Questionnaires \cite{Ashoori2019InProcesses, Chen2005TrustAgents}; Willingness to accept AI agent advice \cite{Hsiao2021RoadmapXAI} \\
  \bottomrule
  \end{tabularx}

  

==> tables/metrics/MetricsFormat.tex <==
\begin{tabularx}{\linewidth}{@{}p{3.5cm}X@{}}
  \toprule
  \textbf{Explanation property} & Measurement \\  \\
  \midrule

  Correctness &  Percentage of invalid rules \cite{Vilone2021NotionsIntelligence} \\

  Completeness &  Rules redundancy \cite{Vilone2021NotionsIntelligence} \\
\hline
 Form of cognitive chunks & BLEU and METEOR \cite{Vilone2021NotionsIntelligence}; Perceptual Realism \cite{Nauta2022FromAI}  \\
   
  \bottomrule
\end{tabularx}

==> tables/metrics/MetricsGeneration.tex <==
\begin{tabularx}{\linewidth}{@{}p{3.5cm}X@{}}
  \toprule
  \textbf{Explanation property} & Generation  \\
  \midrule
  
  AI Model performance & Measured by the model type appropriate metrics: accuracy, f-score, precision, recall and others. \\
  
 AI Model certainty &  This property can be measured for each individual prediction and the global model. If it is measured globally, it should be measured over a dataset similar to the data the real system will face. \cite{Coroama2022EvaluationXAI} \\
     

  Consistency & Implementation invariance: check whether the XAI function parameters are the same after different runs of the XAI method creation \cite{Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence}  \\
  \hline
    Correctness &  Translucency \cite{Carvalho2019MachineMetrics}\\
  \bottomrule
\end{tabularx}


==> tables/metrics/byCC/MetricsExplanationAspects.tex <==
\begin{tabularx}{\linewidth}{@{}XXXXX@{}}
  \toprule
  \textbf{Explanation property} & Generation & Abstraction & Format & Communication \\  \\
  \midrule
  
  Necessity & & Responsability of an outcome \cite{Miller2019}, Sparsity and Sparsity rate \cite{Moreira2022BenchmarkingBox}, Deletion Check \cite{Nauta2022FromAI, Li2022AMetrics} & & \\

  Sufficiency & & Count whether the AI model prediction changes when the non-selected causes change \cite{Miller2019}  & & \\
  
  Correctness &  Translucency \cite{Carvalho2019MachineMetrics} & Model Parameter Randomization Check, Explanation Randomization, White Box Check, Controlled Synthetic Data Check, Predictive Performance \cite{Nauta2022FromAI}, Fidelity  \cite{Sokol2020ExplainabilityApproaches, Coroama2022EvaluationXAI, Nauta2022FromAI}; Alignment between AI model features and explanation features \cite{Li2022AMetrics, Velmurugan2021DevelopingLearning}& Percentage of invalid rules \cite{Vilone2021NotionsIntelligence} & \\

  Completeness & & Preservation Check \cite{Nauta2022FromAI}, Completeness \cite{Coroama2022EvaluationXAI, MoraffahCausalEvaluation}, Recall \cite{Velmurugan2021DevelopingLearning} & Rules redundancy \cite{Vilone2021NotionsIntelligence} & \\

  Contrastivity & & Data Randomization, Target Sensitivity, Target Dicriminativeness \cite{Nauta2022FromAI}; Sensitivity \cite{Vilone2021NotionsIntelligence} & &\\

  Size & & Total size or sparsity \cite{Nauta2022FromAI} & &\\
  
  Structure & & Incremental Deletion \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Covariate Regularity \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Chronology \cite{Sokol2020ExplainabilityApproaches}; Single Deletion \cite{Nauta2022FromAI} &   &  Questionnaire \cite{Vilone2021NotionsIntelligence, Chen2005TrustAgents} \\

  Representativeness & & Explanation support (number of instances to which the explanation applies over the number of instances) \cite{Sokol2020ExplainabilityApproaches, Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence, Coroama2022EvaluationXAI}& & \\
   
  \bottomrule
\end{tabularx}

==> tables/metrics/byCC/MetricsExplanationAspects2.tex <==
\begin{tabularx}{\linewidth}{@{}XXXX@{}}
  \toprule
  \textbf{Explanation property} & Generation &  Format & Communication \\  \\
  \midrule
  
  Necessity & & & \\

  Sufficiency & & & \\
  
  Correctness &  Translucency \cite{Carvalho2019MachineMetrics}  & Percentage of invalid rules \cite{Vilone2021NotionsIntelligence} & \\

  Completeness & & Rules redundancy \cite{Vilone2021NotionsIntelligence} & \\

  Contrastivity & & &\\

  Size & & &\\
  
  Structure & &  &  Questionnaire \cite{Vilone2021NotionsIntelligence, Chen2005TrustAgents} \\

  Representativeness & & & \\
   
  \bottomrule
\end{tabularx}

\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \textbf{Explanation property} & Abstraction \\
  \midrule
  
  Necessity & Responsability of an outcome \cite{Miller2019}; Sparsity and Sparsity rate \cite{Moreira2022BenchmarkingBox}; Deletion Check \cite{Nauta2022FromAI, Li2022AMetrics} \\

  Sufficiency & Count whether the AI model prediction changes when the non-selected causes change \cite{Miller2019} \\
  
  Correctness &  Model Parameter Randomization Check, Explanation Randomization, White Box Check, Controlled Synthetic Data Check, Predictive Performance \cite{Nauta2022FromAI}; Fidelity  \cite{Sokol2020ExplainabilityApproaches, Coroama2022EvaluationXAI, Nauta2022FromAI}; Alignment between AI model features and explanation features \cite{Li2022AMetrics, Velmurugan2021DevelopingLearning}\\

  Completeness & Preservation Check \cite{Nauta2022FromAI}; Completeness \cite{Coroama2022EvaluationXAI, MoraffahCausalEvaluation}; Recall \cite{Velmurugan2021DevelopingLearning}  \\

  Contrastivity & Data Randomization, Target Sensitivity, Target Dicriminativeness \cite{Nauta2022FromAI}; Sensitivity \cite{Vilone2021NotionsIntelligence} \\

  Size & Total size or sparsity \cite{Nauta2022FromAI} \\
  
  Structure & Incremental Deletion \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Covariate Regularity \cite{Nauta2022FromAI, Coroama2022EvaluationXAI}; Chronology \cite{Sokol2020ExplainabilityApproaches}; Single Deletion \cite{Nauta2022FromAI} \\

  Representativeness & Explanation support (number of instances to which the explanation applies over the number of instances) \cite{Sokol2020ExplainabilityApproaches, Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence, Coroama2022EvaluationXAI} \\
   
  \bottomrule
\end{tabularx}

==> tables/metrics/byCC/MetricsInteraction.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Communication of explanation}   \\
  \midrule
    Efficiency & Interaction time and number of interactions to perform a task \cite{Tintarev2015ExplainingEvaluation}\\
    
    Performance & Performance metrics with respect to the primary goal \cite{Hoffman2018MetricsProspects} \\
    
    Reliance & Questionnaires \cite{Ashoori2019InProcesses, Chen2005TrustAgents}; Willingness to accept AI agent advice \cite{Hsiao2021RoadmapXAI} \\

    \bottomrule
\end{tabularx}


==> tables/metrics/byCC/MetricsObjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}lXXX@{}}
  \toprule
  \textbf{Explanation property} & Generation & Abstraction \\
  \midrule
  
  Model performance & Measured by the model type appropriate metrics: accuracy, f-score, precision, recall and others. & \\
  
  Model certainty &  This property can be measured for each individual prediction and the global model. If it is measured globally, it should be measured over a dataset similar to the data the real system will face. \cite{Coroama2022EvaluationXAI} & \\
  
  Certainty & Confidence Accuracy \cite{Nauta2022FromAI} &  \\
   
  Continuity & & Connectedness \cite{Nauta2022FromAI} also in \cite{Singh2022ExplainabilityMethods, MoraffahCausalEvaluation, Moreira2022BenchmarkingBox, Vilone2021NotionsIntelligence, Ge2021CounterfactualAI, Carlevaro2022CounterfactualDescription}; Stability for Slight Variations \cite{Nauta2022FromAI}; Fidelity for Slight Variations \cite{Nauta2022FromAI}  \\

  Separability & & Separability \cite{Carvalho2019MachineMetrics} \\

  Consistency & Implementation invariance: check whether the XAI function parameters are the same after different runs of the XAI method creation \cite{Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence} & Stability of explanation: check whether the explanations for a single object change for different instances of the XAI method \cite{Coroama2022EvaluationXAI, Carvalho2019MachineMetrics} \\

  \bottomrule
\end{tabularx}


==> tables/metrics/byCC/MetricsSubjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}XXXXX@{}}
  \toprule
  \textbf{Explanation property} & Abstraction & Format & Communication \\  \\
  \midrule
    Explanation power & Sensitivity Axiom \cite{Carvalho2019MachineMetrics} & & Questionnaire \cite{Vilone2022AIntelligence}\\

    Form of cognitive chunks & Covariate Homogeneity \cite{Nauta2022FromAI} & BLEU and METEOR \cite{Vilone2021NotionsIntelligence}; Perceptual Realism \cite{Nauta2022FromAI} & Perceived Homogeneity \cite{Nauta2022FromAI} \\

    Information expectedness & Alignment with Domain Knowledge \cite{Nauta2022FromAI} & &  Questionnaire \cite{Vilone2022AIntelligence}\\
    
    Perceived model competence & & & Questionnaire \cite{Ashoori2019InProcesses}\\

    Cognitive Load & & &  NASA TLX \cite{Hsiao2021RoadmapXAI}\\
   
    Relevance to the task & Pragmatism \cite{Nauta2022FromAI, Coroama2022EvaluationXAI, Moreira2022BenchmarkingBox}; Attribute costs \cite{Vilone2021NotionsIntelligence} & & Questionnaire \cite{Vilone2022AIntelligence}\\
    
    Alignment with situational context & & &  Goodness explanation \cite{Hoffman2018MetricsProspects} \\
\bottomrule
 \end{tabularx}



==> tables/metrics/byCC/MetricsUserExperience.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \textbf{Explanation property} & Communication \\  \\
  \midrule
    Curiosity & Curiosity Checklist \cite{Hoffman2018MetricsProspects}; Eye Movement Pattern \cite{Hsiao2021RoadmapXAI} \\

    Satisfaction & Explanation Satisfaction Scale \cite{Hoffman2018MetricsProspects}; Eye Movement Pattern \cite{Hsiao2021RoadmapXAI}; Loyalty \cite{Tintarev2015ExplainingEvaluation}; Questionnaire \cite{Ashoori2019InProcesses} \\
  
    Trust & Trust Scale \cite{Hoffman2018MetricsProspects}; Questionnaire \cite{Ashoori2019InProcesses, Chen2005TrustAgents, Pu2007Trust-inspiringSystems, Vilone2022AIntelligence}\\

    Understanding & Questionnaires \cite{Tintarev2015ExplainingEvaluation,Ashoori2019InProcesses, Vilone2022AIntelligence}\\

    Helpfulness & Questionnaires \cite{Tintarev2015ExplainingEvaluation, Vilone2022AIntelligence}; Evaluate user action before and after explanation \cite{Tintarev2015ExplainingEvaluation}\\

    Controllability & Concept-level feedback Satisfaction Ratio \cite{Chen2020TowardsRecommendation}; The extent to which a user can produce certain outcomes \cite{Hoffman2018MetricsProspects}\\
  \bottomrule
  \end{tabularx}

  

==> tables/properties/PropertiesExplanationAspects.tex <==
\begin{tabularx}{\linewidth}{@{}lXX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Definition}  & \textbf{Related work}  \\
  \midrule
 Necessity & Measures whether the explanation method selected the causes that are responsible for the prediction. If the necessary causes change, then the prediction will also change.  & \cite{Miller2019, Liao2022ConnectingAI, Nauta2022FromAI, Carvalho2019MachineMetrics} \\

  Sufficiency & 
  Measures whether the explanation method did not select causes that do not affect the prediction. If non-selected causes change, the prediction would still hold, and thus the explanation should not change. & \cite{Miller2019} \\

  Correctness &  Quantifies the extent to which the selected causes are correct with respect to the model reasoning
   & \cite{Liao2022ConnectingAI, Carvalho2019MachineMetrics, Nauta2022FromAI, Markus2020TheStrategies, Vilone2021NotionsIntelligence, Sokol2020ExplainabilityApproaches} \\

  Completeness & Quantifies if all the causes that the model used to generate the prediction are present in the explanation. & \cite{Carvalho2019MachineMetrics, Nauta2022FromAI, Liao2022ConnectingAI, Markus2020TheStrategies, Vilone2021NotionsIntelligence} \\

  Contrastivity & Measures whether the explanation contains reasons that highlight differences with respect to other possible outcomes. Low contrastivity will provide the same reasons for instances in which the model predicts different classes. & \cite{Carvalho2019MachineMetrics, Nauta2022FromAI, Miller2019} \\

  Size & Refers to the amount of information present in the explanation. & \cite{Nauta2022FromAI, Carvalho2019MachineMetrics, Vilone2021NotionsIntelligence, Markus2020TheStrategies, Liao2022ConnectingAI, Doshi-Velez2017TowardsLearning} \\
  
  Structure & The information should be displayed in a way that allows the users to understand the hierarchy of the information quickly & \cite{Nauta2022FromAI, Hsiao2021RoadmapXAI, Carvalho2019MachineMetrics, Tonekaboni2019WhatUse, Tintarev2015ExplainingEvaluation, Markus2020TheStrategies, Vilone2021NotionsIntelligence, Sokol2020ExplainabilityApproaches} \\

  Representativeness & An explanation is representative if it holds for many distinct but similar instances. & \cite{Carvalho2019MachineMetrics, Coroama2022EvaluationXAI, Vilone2021NotionsIntelligence, Sokol2020ExplainabilityApproaches} \\
   
  \bottomrule
\end{tabularx}



==> tables/properties/PropertiesInteraction.tex <==
\begin{tabularx}{\linewidth}{@{}lXX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Definition}  & \textbf{Related work}  \\
  \midrule
    Efficiency & Measures the speed at which a task can be performed. & \cite{Vilone2021NotionsIntelligence, Tintarev2015ExplainingEvaluation}\\
    
    Performance & Measures how well the user can do the task while using the system (prediction+explanations). & \cite{Lofstrom2022AMethods, Hsiao2021RoadmapXAI, Hoffman2018MetricsProspects} \\
    
    Reliance & Measures whether the user is willing to provide control to the machine for the given task. & \cite{Hoffman2018MetricsProspects, Hsiao2021RoadmapXAI, Tintarev2015ExplainingEvaluation, Vilone2021NotionsIntelligence} \\

    \bottomrule
\end{tabularx}


==> tables/properties/PropertiesObjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}XXX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Definition}  & \textbf{Related work}                                        \\
  \midrule
  AI Model performance
  & The accomplishment level the AI model has with respect to the task for which it was trained.  
  & \\
  
  AI Model certainty
  & The confidence the AI model has in its prediction.  
  & \cite{Liao2022ConnectingAI,Carvalho2019MachineMetrics,Nauta2022FromAI, Vilone2021NotionsIntelligence} \\

  Certainty  
  & The confidence the XAI method has in the explanation. 
  & \cite{Hoffman2018MetricsProspects, Carvalho2019MachineMetrics, Nauta2022FromAI, Liao2022ConnectingAI, Beckh2022ALearning, Tintarev2015ExplainingEvaluation}\\
  
  Continuity 
  & The function should be smooth to provide similar explanations for similar instances. 
  & \cite{Hsiao2021RoadmapXAI, Coroama2022EvaluationXAI, Hoffman2018MetricsProspects, Carvalho2019MachineMetrics, Markus2020TheStrategies} \\
  
  Separability & The XAI method should return different explanations for different instances. & \cite{Carvalho2019MachineMetrics}\\
  
  Consistency 
  & The degree to which different runs of the XAI method yield similar XAI functions.
  & \cite{Hsiao2021RoadmapXAI, Carvalho2019MachineMetrics, Nauta2022FromAI, Tonekaboni2019WhatUse, Liao2022ConnectingAI, Vilone2021NotionsIntelligence, Beckh2022ALearning, Lofstrom2022AMethods}\\
    
  \bottomrule
\end{tabularx}


==> tables/properties/PropertiesSubjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}XXX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Definition}  & \textbf{Related work}  \\
  \midrule
    Explanation power & Measures whether the selected causes make the user understand the reasons the model considered when making a decision & \cite{Liao2022ConnectingAI, Vilone2021NotionsIntelligence, Carvalho2019MachineMetrics, Wanner2022ALearning} \\

    Form of cognitive chunks & Refers to the semantics and structure of the pieces of information the user will receive. & \cite{Doshi-Velez2017TowardsLearning, Nauta2022FromAI, Vilone2021NotionsIntelligence, Carvalho2019MachineMetrics}\\

    Information expectedness & Level of surprise of the information revealed by the explanation & \cite{Hsiao2021RoadmapXAI, Carvalho2019MachineMetrics,Nauta2022FromAI, Tonekaboni2019WhatUse, Miller2019, Liao2022ConnectingAI, Vilone2021NotionsIntelligence, Sokol2020ExplainabilityApproaches, Beckh2022ALearning, MoraffahCausalEvaluation,Lofstrom2022AMethods, Moreira2022BenchmarkingBox}\\
    
    Perceived model competence & Measures the user's impression of the model competence for the task at hand & \cite{Chen2005TrustAgents} \\

    Cognitive Load & Refers to the cognitive effort the user has to do to achieve the task. & \cite{Carvalho2019MachineMetrics, Liao2022ConnectingAI, Vilone2021NotionsIntelligence}\\
   
    Relevance to the task & Level of explanation usefulness to the user's task. & \cite{Hsiao2021RoadmapXAI, Nauta2022FromAI, Tonekaboni2019WhatUse, Miller2019, Liao2022ConnectingAI, Vilone2021NotionsIntelligence, Moreira2022BenchmarkingBox, Wanner2022ALearning}  \\
    
    Alignment with situational context & Level of appropriateness of the explanation to the usage context& \cite{Hsiao2021RoadmapXAI, Carvalho2019MachineMetrics, Tonekaboni2019WhatUse, Liao2022ConnectingAI, Sokol2020ExplainabilityApproaches}\\
\bottomrule
  \end{tabularx}



==> tables/properties/PropertiesUserExperience.tex <==
\begin{tabularx}{\linewidth}{@{}lXX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Definition}  & \textbf{Related work}  \\
  \midrule
    Curiosity &  Measures whether the user is intrinsically motivated to understand the explanation. If the user is curious, she will be more attentive to the task and, therefore, more engaged with the system. & \cite{Hoffman2018MetricsProspects, Vilone2021NotionsIntelligence, Hsiao2021RoadmapXAI} \\

    Satisfaction & Refers to the level of fulfilment the user gets while interacting with the system. This satisfaction is always measured at the communication level because it is for the users to decide whether they feel good about the overall system interaction. & \cite{Hsiao2021RoadmapXAI, Hoffman2018MetricsProspects, Tintarev2015ExplainingEvaluation, Vilone2021NotionsIntelligence, Wanner2022ALearning}\\
  
    Trust & We use \citet{Tintarev2015ExplainingEvaluation} definition :"perceived confidence in a system's competence" &  \cite{Hsiao2021RoadmapXAI, Hoffman2018MetricsProspects, Tonekaboni2019WhatUse, Liao2022ConnectingAI, Tintarev2015ExplainingEvaluation, Chen2005TrustAgents, Ashoori2019InProcesses, Wanner2022ALearning} \\

    Understanding & Refers to the ability of the user to interpret the system's output correctly. The user will fail to understand when she cannot interpret or incorrectly interprets the system's explanation and prediction. This involves the creation of the user's mental model and how that aligns with the system's functionality. & \cite{Carvalho2019MachineMetrics,  Hoffman2018MetricsProspects, Hsiao2021RoadmapXAI, Lofstrom2022AMethods, Markus2020TheStrategies, Vilone2021NotionsIntelligence, Wanner2022ALearning}\\

    Usefulness & Measures whether the explanation helps the user to understand the prediction made by the AI model.  & \cite{Beckh2022ALearning, Tintarev2015ExplainingEvaluation, Vilone2021NotionsIntelligence, Wanner2022ALearning} \\

    Controllability & Measures whether the user perceives she has some level of control over the system. This could manifest as the ability to reverse actions, correct the system, filter or zoom the explanation, or ask questions to clarify the explanation or prediction. & \cite{Hoffman2018MetricsProspects, Hsiao2021RoadmapXAI, Liao2022ConnectingAI, Nauta2022FromAI, Sokol2020ExplainabilityApproaches, Tintarev2015ExplainingEvaluation, Vilone2021NotionsIntelligence}\\
  \bottomrule
  \end{tabularx}



==> tables/relations/RelationsExplanationAspects.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
    \textbf{Explanation property} & \textbf{Relation to other metrics}
  \\
  \midrule
  
  Necessity & The explanation power depends on the quality of the selected causes, which is measured by the sufficiency, necessity \cite{Liao2022ConnectingAI} and constrastivity properties.\\

  Sufficiency & The explanation power depends on the quality of the selected causes, which is measured by the sufficiency, necessity \cite{Liao2022ConnectingAI} and constrastivity properties.\\

  Correctness & An explanation with high correctness will faithfully reflect the decision process of the AI model. This could increase Trust in the explanation and AI model \\

  Completeness & The explanation size is related to completeness: the bigger the explanation, the more complete it will be \cite{Liao2022ConnectingAI, Carvalho2019MachineMetrics}. However, bigger explanations might decrease curiosity \cite{Hsiao2021RoadmapXAI}. \\

  Contrastivity & The explanation power depends on the quality of the selected causes, which is measured by the sufficiency, necessity \cite{Liao2022ConnectingAI} and constrastivity properties. Additionally, this property will affect understanding because the people expect explanations to be contrastive \cite{Miller2019}. \\

  Size & The amount of information affects curiosity in an inverted U-shaped pattern: little or excessive information reduces curiosity \cite{Hsiao2021RoadmapXAI}. The size of the explanation also affects how easily a user can understand the explanation \cite{Liao2022ConnectingAI, Markus2020TheStrategies}. This last effect could be mediated by the Cognitive Load.\\
  
  Structure & The design of the information that will be shown affects its trustworthiness \cite{Tintarev2015ExplainingEvaluation}, curiosity \cite{Hsiao2021RoadmapXAI} and ultimately how easy they can be understood \cite{Markus2020TheStrategies, Sokol2020ExplainabilityApproaches}.  \\

  Representativeness & This property affects understanding, cognitive load and efficiency because the user can understand more quickly an explanation if it is similar to ones she has seen before. \\
   
  \bottomrule
\end{tabularx}






==> tables/relations/RelationsObjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Relation to other metrics}
  \\
  \midrule
  Model performance
  & The performance of the AI will affect the level of Trust the users can achieve \cite{Tintarev2015ExplainingEvaluation, Dominguez2019} \\
  
  Model certainty
  & If the AI model is uncertain of the predictions, the XAI method will have more difficulties obtaining consistent explanations, which will affect the XAI method's certainty. This confidence will also affect the satisfaction with the system because, as \citet{Tintarev2015ExplainingEvaluation} explains, a user might be more forgiving if the system admits it is not confident about a prediction.\\

  Certainty & If the explanation shows its limitations, the user may not relay or trust the system \cite{Hoffman2018MetricsProspects, Liao2022ConnectingAI}. Low certainty will affect the correctness of the explanation.\\
  
  Continuity & Higher continuity increases the understanding of the model because the similarity of explanations helps to learn from the model. It also helps to produce contrastive and representative explanations. Ultimately, high continuity can also increase Trust \cite{Tonekaboni2019WhatUse}.\\
  
  Separability & Higher separability increases the understanding of the model and the contrastivity of the explanations. \\
  
  Consistency & Low consistency may decrease user satisfaction \cite{Hsiao2021RoadmapXAI} and correctness \cite{Liao2022ConnectingAI}\\
  
  
  \bottomrule
\end{tabularx}

==> tables/relations/RelationsSubjectiveSystemAspects.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \textbf{Explanation property} & \textbf{Relation to other metrics}
  \\
  \midrule
     Explanation power & The quality of the causes selected will help to increase understanding. \\

    Form of cognitive chunks &  It affects understanding because this property measures how interpretable are the information pieces the user receives \cite{Carvalho2019MachineMetrics} \\

    Information expectedness & If the information is coherent with the user's beliefs, they will be more likely to understand it \cite{Sokol2020ExplainabilityApproaches}. However, if the information does not add anything new to their existing knowledge, they are less likely to be curious \cite{Sokol2020ExplainabilityApproaches}.   \\
    
    Perceived model competence & When the users perceive the AI model can perform, they are more likely to trust it and eventually to rely on it \cite{Chen2005TrustAgents}.\\

    Cognitive Load & An explanation with low cognitive load will be easier to understand \cite{Liao2022ConnectingAI}.\\
   
    Relevance to the task & If the explanations help the development of the task, the user is more likely to rely on the AI advice. \\
    
    Alignment with situational context & Trust in the system is context-dependent. If the system is aligned with the situation the user has to perform, she will be more likely to trust it. \cite{Hoffman2018MetricsProspects}. Additionally, this could build up until the user starts to rely on the AI agent.\\
\bottomrule
  \end{tabularx}


==> tables/relations/RelationsUserExperience.tex <==
\begin{tabularx}{\linewidth}{@{}lX@{}}
  \toprule
  \\textbf{Explanation property} & \textbf{Relation to other metrics}  \\
  \midrule
    Curiosity & Mental model formation, which is the final goal of understanding, is modulated by Curiosity \cite{Hsiao2021RoadmapXAI}. Additionally, Curiosity encourages users to explore and interact with the system \cite{Hsiao2021RoadmapXAI}.  \\

    Satisfaction & \\
  
    Trust & Reliance is an outcome of appropriate trust \cite{Tintarev2015ExplainingEvaluation, Hsiao2021RoadmapXAI, Chen2005TrustAgents, Hoffman2018MetricsProspects}. Mental model formation is also modulated by Trust in the system \cite{Hsiao2021RoadmapXAI}\\

    Understanding & If users cannot understand the behaviour, Trust will be lost \cite{Hsiao2021RoadmapXAI}\\

    Helpfulness & If the user finds the explanations helpful, they are more likely to increase the user performance with the system.\\

    Controllability & The possibility of interaction increases Trust in the system \cite{Tintarev2015ExplainingEvaluation}. Good interaction with the system can increase the performance of the users \cite{Hsiao2021RoadmapXAI}\\
  \bottomrule
  \end{tabularx}

  
